Optimal Shallow Circuits for Majority

Four decades on, H{\aa}stad's classical $2^{\Omega(n^{1/(d-1)})}$ lower bound for depth-$d$ circuits computing Parity remains the best known $\mathrm{AC}^0$ circuit lower bound for any explicit function. Majority has long been a compelling candidate for stronger lower bounds: the most natural circuits computing it are substantially larger than those for Parity and have repeatedly been conjectured to be optimal. We present a simple construction, found by GPT-6 Astra, of depth-$d$ circuits of size $2^{O(n^{1/(d-1)})}$ for any symmetric function. This result settles the asymptotic $\mathrm{AC}^0$ circuit complexity of Majority, matching H{\aa}stad's lower bound. The proof draws inspiration from well-loved combinatorial tools, including the color-coding technique of Alon, Yuster, and Zwick (1995).

==> figures/circuit-negations-base.tex <==
\begingroup%
\def\circuitHeightDivisor{4}%
\def\circuitInputBits{{1,1,0,0,1,0,0,0,1,0,0,0,1,0,0,1}}%
\def\circuitBottomInputs{{{1,2,3,5},{1,3,4,5},{3,4,-6,7},{7,8,-9,10},{7,-10,11,12},{9,11,12,14},{12,-13,14,15},{12,13,14,16}}}%
\def\circuitMiddleInputs{{{1,2,4},{1,2,3},{2,5,6},{6,7,8},{5,6,8}}}%
\def\circuitMarkerPositions{{0.50,0.50,0.45,0.37,0.45,0.50,0.45,0.50}}%
\definecolor{circuitGreen}{HTML}{D6EBD8}%
\definecolor{circuitInk}{HTML}{34423C}%
\definecolor{circuitWire}{HTML}{87928B}%
\pgfmathsetlengthmacro{\circuitWidth}{\linewidth}%
\pgfmathsetlengthmacro{\circuitHeight}{\linewidth/\circuitHeightDivisor}%
\pgfmathsetmacro{\circuitEndInset}{max(0.06,3mm/\circuitHeight)}%
\pgfmathtruncatemacro{\circuitInputCount}{dim(\circuitInputBits)}%
\pgfmathtruncatemacro{\circuitBottomCount}{dim(\circuitBottomInputs)}%
\pgfmathtruncatemacro{\circuitMiddleCount}{dim(\circuitMiddleInputs)}%
\begin{tikzpicture}[
  x=\circuitWidth,
  y=\circuitHeight,
  font=\fontsize{11}{13}\selectfont,
  circuit/node/.style={draw=circuitInk, text=circuitInk, line width=0.55pt, inner sep=0pt, outer sep=0pt, fill=white},
  circuit/input/.style={circuit/node, rectangle, minimum size=4.8mm},
  circuit/gate/.style={circuit/node, circle, minimum size=5.4mm},
  circuit/inversion/.style={circuit/node, circle, minimum size=\circuitInversionSize, font=\fontsize{8}{8}\selectfont},
  circuit/state/.is choice,
  circuit/state/0/.style={fill=white},
  circuit/state/1/.style={fill=circuitGreen},
  circuit/wire/.style={draw=circuitWire, line width=0.4pt, -{Stealth[length=1.35mm,width=1.0mm]}, shorten <=0.3pt, shorten >=0.3pt},
  declare function={
    circuitbit(\i)=\circuitInputBits[\i-1];
    circuitliteral(\i)=abs(circuitbit(abs(\i))-(\i<0));
    circuitor(\i)=max(circuitliteral(\circuitBottomInputs[\i-1][0]),circuitliteral(\circuitBottomInputs[\i-1][1]),circuitliteral(\circuitBottomInputs[\i-1][2]),circuitliteral(\circuitBottomInputs[\i-1][3]));
    circuitand(\i)=min(circuitor(\circuitMiddleInputs[\i-1][0]),circuitor(\circuitMiddleInputs[\i-1][1]),circuitor(\circuitMiddleInputs[\i-1][2]));
  }
]
  \path[use as bounding box] (0,0) rectangle (1,1);

  \foreach \i in {1,...,\circuitInputCount} {
    \pgfmathtruncatemacro{\value}{circuitbit(\i)}
    \node[circuit/input, circuit/state=\value] (input-\i) at ({(\i-0.5)/\circuitInputCount},\circuitEndInset) {$\value$};
  }
  \foreach \i in {1,...,\circuitBottomCount} {
    \pgfmathtruncatemacro{\value}{circuitor(\i)}
    \node[circuit/gate, circuit/state=\value] (bottom-\i) at ({0.04+0.92*(\i-0.5)/\circuitBottomCount},0.35) {$\vee$};
  }
  \foreach \i [remember=\outputValue as \previousOutput (initially 0)] in {1,...,\circuitMiddleCount} {
    \pgfmathtruncatemacro{\value}{circuitand(\i)}
    \pgfmathtruncatemacro{\outputValue}{max(\previousOutput,\value)}
    \node[circuit/gate, circuit/state=\value] (middle-\i) at ({0.10+0.80*(\i-0.5)/\circuitMiddleCount},0.65) {$\wedge$};
    \ifnum\i=\circuitMiddleCount
      \node[circuit/gate, circuit/state=\outputValue] (output) at (0.5,{1-\circuitEndInset}) {$\vee$};
    \fi
  }

  \begin{scope}[on background layer]
    \foreach \i in {1,...,\circuitBottomCount} {
      \foreach \j in {0,...,3} {
        \pgfmathtruncatemacro{\source}{abs(\circuitBottomInputs[\i-1][\j])}
        \draw[circuit/wire] (input-\source) -- (bottom-\i);
      }
    }
    \foreach \i in {1,...,\circuitMiddleCount} {
      \foreach \j in {0,...,2} {
        \pgfmathtruncatemacro{\source}{\circuitMiddleInputs[\i-1][\j]}
        \draw[circuit/wire] (bottom-\source) -- (middle-\i);
      }
      \draw[circuit/wire] (middle-\i) -- (output);
    }
  \end{scope}
  \foreach \i in {1,...,\circuitBottomCount} {
    \foreach \j in {0,...,3} {
      \pgfmathtruncatemacro{\literal}{\circuitBottomInputs[\i-1][\j]}
      \ifnum\literal<0
        \pgfmathtruncatemacro{\source}{abs(\literal)}
        \pgfmathsetmacro{\markerPosition}{\circuitMarkerPositions[\i-1]}
        \path (input-\source.center) -- (bottom-\i.center) node[pos=\markerPosition, circuit/inversion] {$\circuitInversionSymbol$};
      \fi
    }
  }
\end{tikzpicture}%
\endgroup%

